Keeping Authorities "Honest or Bust" with Decentralized Witness Cosigning

The secret keys of critical network authorities - such as time, name, certificate, and software update services - represent high-value targets for hackers, criminals, and spy agencies wishing to use these keys secretly to compromise other hosts. To protect authorities and their clients proactively from undetected exploits and misuse, we introduce CoSi, a scalable witness cosigning protocol ensuring that every authoritative statement is validated and publicly logged by a diverse group of witnesses before any client will accept it. A statement S collectively signed by W witnesses assures clients that S has been seen, and not immediately found erroneous, by those W observers. Even if S is compromised in a fashion not readily detectable by the witnesses, CoSi still guarantees S's exposure to public scrutiny, forcing secrecy-minded attackers to risk that the compromise will soon be detected by one of the W witnesses. Because clients can verify collective signatures efficiently without communication, CoSi protects clients' privacy, and offers the first transparency mechanism effective against persistent man-in-the-middle attackers who control a victim's Internet access, the authority's secret key, and several witnesses' secret keys. CoSi builds on existing cryptographic multisignature methods, scaling them to support thousands of witnesses via signature aggregation over efficient communication trees. A working prototype demonstrates CoSi in the context of timestamping and logging authorities, enabling groups of over 8,000 distributed witnesses to cosign authoritative statements in under two seconds.

==> contrib.tex <==
\subsection{Contributory Signing Protocol} %Aggregation Protocol?
\label{sec:contrib}

\xxx{Probably delete this subsection,
	subsuming it into the prototype applications.}

%\xxx{Reviewer A: how can a leaf node verify that its own input
%	made it into the aggregate? Inclusion proofs consisting of the Merkle tree components .  --- addressed}
	 

\xxx{the aggregation mode is not clear. it looks
like the leader could just add a non-random number to cancel out all of
the randomness. 

True - if the leader is the last one to add its contribution and he sees 
everyone else's contribution, he can choose his accordingly. 
It doesn't really matter what the leader add since the main goal
of the aggregation protocol is to combine everyone's (generic) input. 
For randomness, yes, the leader the bias the output. 
But the aggregation mode: contribute, validate, aggregate, sign. }

We now relax the simplifying assumption that only the leader 
proposes values to sign. Signers can use \app 
in an {\em contributory} fashion such that the resulting signature is 
on a cryptographic summary of items proposed by all signers.

The \app protocol works like before, but the message $S$ now
corresponds to the top of a Merkle tree built on potentially
application-specific contributions from all signers.
The signers build the Merkle tree of contributions in a bottom-up process
following a leader announcement of a new round. 
Each signer proposes its contribution, hashes %combines 
it with the contributions received from its children and passes it upward
to its parent who repeats the process until it reaches the leader (the top of the Merkle tree).
In response, the leader adds its own contribution which results in a top hash --- a cryptographic 
summary of all items propagated throughout the tree. Finally, the leader
passes down the top hash along with a {\em inclusion proof} consisting of the proper components of
the Merkle tree that he properly incorporated 
the children's contributions. 
In turn, each signer repeats the process until each node in the tree receives 
the top hash and its own inclusion proof that its contribution was included and 
therefore witnessed by other signers. 

Application semantics determine how signers
combine their contributions during this process. 
In an {\em aggregation mode}, each signer proposes a unique value,
which is aggregated into a single, collective value that is a function
of each signer's input. This mode is useful for generating
cryptographic random numbers or voting, for example.
In a {\em logging mode}, each signer's proposed contribution is opaque 
to others, consisting of a hash of a single or many values
(\eg, consisting of items its clients requested to log or time-stamp). 
Each signer's signature represents an acknowledgment 
that a particular contribution was indeed seen and merged together.
This mode, in fact, becomes a mechanism for tamper-evident logging. 
A {\em validation mode} gives each signer an opportunity to view and validate
other signer's contributions and withhold its signature, raising an alarm 
and alerting others to a potential wrongdoing,  
if some contribution is invalid according to application-specific checks.
Therefore, the collective signature not only conveys that each contribution was 
seen at a particular time but also that it was validated by each signer. 
While this is the most expensive mode with $O(N)$ as opposed to 
$O(\log n)$ cost, it gives signers a unique ability to enforce 
even fine-grain correctness checks. For example, if applied to 
Certificate Transparency, each signer could verify the newly proposed batch 
of certificates to ensure that they are valid and also endorsed by authorized 
entities. 

Regardless of the contributory mode the signers use for \app, each signer only 
contributes its signature share if the resulting top hash is valid
with respect to the specific requirements of each mode.

%Aggregation mode: contribute, validate, aggregate, sign. 



==> elec.tex <==
\subsection{Leader Failures and View Changes}
\label{sec:elec}

%\xxx{	Clarify if/how view changes can handle the case of
%DoS attacks by nodes high up in the tree that dominate many others in the tree. 
%Discuss mechanism for bypassing failed nodes while keeping their children included. (Review A) 
%Mention somewhere: SplitStream~\cite{castro03splitstream} approach as one way to deal gracefully with individual offline servers
%who might be close to the root of the tree.
%Also, already a parent can skip an immediate child and go directly to its children or grandchildren...
	
	
\xxx{ B: The protocol for view changes seems reasonable, but the description is not enough to be convincing that it survives a useful set of failures; having a more robust description akin to the description in PBFT, or how view changes happen in an asynchronous network would be useful.
}

So far we have treated the leader as a distinguished role,
and have addressed only signer failures:
if the leader fails the collective will cease operation.
In some applications this may be appropriate,
\eg, if by design statements to be signed originate only from one source
and are to be merely witnessed and validated by the signers.
In other environments, however,
we would prefer the members of a cothority to play symmetric roles,
such that {\em all} servers can contribute to the statements being signed
and a failed leader can be replaced.

We address leader features using a {\em view change} protocol,
a standard technique used in Byzantine agreement
protocols~\cite{castro99practical}.
For a given cothority membership roster,
we use a well-known, deterministic algorithm
to define a schedule of {\em views},
each numbered view selecting one server in the roster as the view's leader.
Given this choice of leader,
the rest of the communication tree for that view
is similarly defined by a well-known, deterministic function
of the cothority roster and the view number.

In each view, all signers expect that view's leader
to initiate and complete collective signing rounds at an established rate.
Any server who decides that the protocol is not making adequate progress
can broadcast a {\em view change} message proposing a larger view number.
As soon as a configured threshold of servers have broadcast view changes
for a new view $v$, the new leader considers $v$ to be active
and commences initiation of \cosi rounds with itself as the root.

To guarantee the agreement property, that no two views can make progress
simultaneously even in the presence of up to $f$ Byzantine nodes,
the view change threshold needs to be $2f+1$ out of $3f+1$ total nodes.
However, not all cothorities may require this agreement property,
and the protocol can function without it.
For example, if a major network-split divides a timestamp cothority
into two or more isolated subsets,
it may be preferable for each subset to be able to survive
and continue making progress,
each under a different leader and producing a temporarily separate timeline,
until the split is healed.
Whether the agreement property is essential or not
depends on the semantics of the cothority.

In our current protocol,
a view change message is individually signed by the server sending it,
so verifying all relevant view change messages
can unfortunately take $O(N)$ time and network bandwidth per node.
This is not a critical issue provided view changes
are needed not needed often,
as we expect,
but this could represent a DoS attack vulnerability in the worst case.
\xxx{	Cite Clements "making BFT tolerate byzantine faults" paper? ~\cite{clement09making}}
We expect that collective signing could be extended to cover
the {\em initiation} of a new view as well as rounds within it,
so a new leader can produce and exhibit a collective signature
as a more compact and efficiently-checkable proof of its leadership,
but we leave this enhancement to future work.

Handling failures of nodes located high in the communication tree 
is necessary to mitigate the effects of potential failures or DoS attacks. 
Since all nodes know the exact topology of the tree, a parent of
a failed node can bypass it reaching directly to its children or grandchildren 
keeping the tree minimally affected by the failure. 
Additionally, failure-handling mechanisms proposed in SplitStream~\cite{castro03splitstream} 
make it possible to gracefully deal with individual offline nodes who 
might be close to the root of the tree.

\com{

reconfigurations, view changes.

Basic version: just like BFT.
View changes when a threshold of nodes time-out and send a
view-change message.

Fancier version:
Two views "active" at any time: one primary, one challenger.
Challenger operators for a fixed time period,
then consensus decides whether challenger becomes primary or expires.
In either case, new challenger picked randomly for next period.

Nodes can also "vote early" if either primary or challenger fails;
a sufficient number of "early votes" triggers an early view change.
}



==> evo.tex <==
\subsection{Witness Cothority Evolution}
\label{sec:evo}

So far we have assumed that
the roster of witnesses attached to an authority's certificate
is static and unchanging,
at least for the lifetime of the particular authority certificate
in which they are listed.
This may be a reasonable assumption provided
the authority picks witnesses whose stability and public key lifetimes
are at least comparable to the authority's own.
Even if one or a few witnesses permanently shut down
in the middle of the authority's certificate lifetime,
that witness's cosignature will simply be absent
in every subsequent statement the authority signs.

Especially if an authority's witness group becomes large, however,
we may desire a way to evolve the witness roster
on shorter timescales than the lifetime of the authority's certificate:
\eg, once or a few times per year rather than once in 3--5 years.
To address this challenge,
the authority can periodically propose, and obtain a collective signature on,
a statement defining a new witness group.
Once collectively signed and published,
the authority immediately starts using the new witness roster
in place of the old one for collective signing.
The new roster may be different not only
in the addition or removal of witnesses,
but also may contain fresh public keys for some or all
existing, stable witnesses,
enabling witnesses to rollover their signing keys more rapidly
for enhanced security.

One challenge is
how clients and other third-parties track and validate
these witness roster changes.
For example, a client application may have a cothority roster
hard-wired into its software,
just as web browsers currently contain hard-wired list of root CAs,
but the cothority's roster may evolve faster
than client software gets updated.

To enable old clients to learn about and validate new \coty rosters,
the client can follow
a chain of collectively-signed roster-change records forward
from the last version it knows about to the current version.
For example, if the client has version $V_0$
and the current roster version is $V_2$,
the client first obtains the change-record from $V_0$ to $V_1$
and validates its signature against the $V_0$ roster,
then obtains the change-record from $V_1$ to $V_2$
and validates its signature against the $V_1$ roster.
So that clients need not pick through a cothority's entire log
to catch up on the latest roster,
a cothority can maintain a separate log containing only roster-change events.

A related issue is how long these forward roster validation chains might become,
but we do not expect this to be a major problem in practice
if roster updates are administratively limited to a reasonable rate,
\eg, by batching all roster changes together at most once per month.

\com{
A relevant question of course is how long these chains might become,
and how quickly they change,
and hence how many forward-version changes a client might need to
``catch up'' on to obtain and validate a cothority's latest roster.

Rate of evolution: might assume moderate, perhaps once a month, once a year?

An alternative that might sometimes work is to form
a kind of ``forward skip-list.''
For example, suppose the cothority roster can change once per day:
thus, a new version record might appear each day,
and a client that hasn't been used in a year or more
might find itself having to dig through hundreds of days'
worth of cothority roster update links.
However, if suppose on the first day of each month,
the previous month's cothority roster signs and validates
a ``new-monthly-roster'' that effectively allows old clients
to skip forward the whole month,
ignoring the daily updates within the month.
Similarly, on the first day of each year,
the cothority represented by the roster that was in effect
on the first day of the previous year collectively signs
a cothority roster update that skips forward by the whole year,
enabling clients with very old state to update them a year at a time.

This skip-forward design obviously offers efficiency benefits,
but does have at least one drawback:
the ``old version'' of a cothority --
\eg, from a month or a year in the past --
must remain operational and (collectively) trustworthy
until its ``long-step'' skip-forward record can be decided on
and collectively signed.
If ``too many'' members of last year's beginning-of-year roster
go permanently offline during the course of this year,
for example,
then it may become impossible for the remaining members
to achieve the required threshold to sign the
yearly-roster-update skip-forward record.
A related downside is that cothority participants
that need to update the roster to refresh their keys
won't be able to fully discard and invalidate their old keys
until at least a full year after the re-keying event,
to ensure that they can still use their old keys to sign
the skip-by-one-year record at the beginning of the next year.
However, these issues are probably surmountable,
given that it is standard practice for long-term CA certificates
to be valid for multiple consecutive years anyway.
}%com

\xxx{	how does the client know that it has the latestview of the roster?}



==> form.tex <==
\com{	I decided the whole epoch idea is problematic and needs to be avoided
	because of the question of how clients validate the temporary
	signing keys for this epoch, etc.  
	So just consider slow cothority evolution instead.

\subsection{Cothority Formation and Identity}

\xxx{ address these low-level crypto details later}

Roster...

A signing policy defines the application it pertains to,
provides the group roster listing all signatories and 
their verified public keys, and defines a
quorum of signatories, that is, the minimum number of noes
whose public keys must be included in the aggregate 
key for the signature created with respect to that key to be valid. 

...

Discrete log keys are vulnerable to related keys attacks, that is, 
a malicious signer can choose his key as a function of other
signers' keys~\cite{XXX}.
To address this issue, before a node can become a signatory, he needs 
to register his public key and prove the knowledge of his secret key. 
Only after the key is successfully verified, the node can join in and participate. 

We assume that each node $i$ has a long-term certified public/secret key pair 
$(Y_i, y_i)$. Node $i$ uses this key during the group formation and joining phase. 
Within \app, however, node $i$ uses its ephemeral public/secret key pair 
$E_i, e_i$, obtaining a fresh ephemeral key pair for each epoch. 

Therefore, at any time \app maintains two rosters: a long-term roster of nodes approved to 
be \app signatories and an ephemeral per-epoch roster of currently active (participating)
signatories.  

Adding signatories can happen in batches. 
After there are enough new requests 
accumulated, they are made available to the current signatories 
(or a designed subset of signatories responsible for group evolution)
and after all keys can be independently verified, they new long term group roster
is collectively signed.   

Each ephemeral roster is refreshed for every epoch and contains a subset of
nodes listed in the long term roster. 
This can be maintained as a look-up table for each $i$ that contains
the long term public key $Y_i$, epoch $j$, ephemeral public key $E^j_i$ 
for epoch $j$, and the proof-of-insurance of $E^j_i$ (see Section~\ref{sub:life}
for the details of the life insurance policy approach).

}%com

